Fair for All: Best-effort Fairness Guarantees for Classification

Standard approaches to group-based notions of fairness, such as \emph{parity} and \emph{equalized odds}, try to equalize absolute measures of performance across known groups (based on race, gender, etc.). Consequently, a group that is inherently harder to classify may hold back the performance on other groups; and no guarantees can be provided for unforeseen groups. Instead, we propose a fairness notion whose guarantee, on each group $g$ in a class $\mathcal{G}$, is relative to the performance of the best classifier on $g$. We apply this notion to broad classes of groups, in particular, where (a) $\mathcal{G}$ consists of all possible groups (subsets) in the data, and (b) $\mathcal{G}$ is more streamlined. For the first setting, which is akin to groups being completely unknown, we devise the {\sc PF} (Proportional Fairness) classifier, which guarantees, on any possible group $g$, an accuracy that is proportional to that of the optimal classifier for $g$, scaled by the relative size of $g$ in the data set. Due to including all possible groups, some of which could be too complex to be relevant, the worst-case theoretical guarantees here have to be proportionally weaker for smaller subsets. For the second setting, we devise the {\sc BeFair} (Best-effort Fair) framework which seeks an accuracy, on every $g \in \mathcal{G}$, which approximates that of the optimal classifier on $g$, independent of the size of $g$. Aiming for such a guarantee results in a non-convex problem, and we design novel techniques to get around this difficulty when $\mathcal{G}$ is the set of linear hypotheses. We test our algorithms on real-world data sets, and present interesting comparative insights on their performance.

==> broader_impact.tex <==
\section*{Broader Impact}
The classification methods presented in this paper are geared towards guaranteeing fairness to all possible groups in the data. Such methods are extremely useful in situations where it is unclear what the protected groups should be. In other cases, when we try to optimize for a certain notion of fairness for some pre-defined groups, questions can be raised about the performance achieved on a group not accounted for beforehand, and thereby lead to complaints from such groups. Our methods can also serve as a baseline to make sure that there is no potential group being unduly affected. The more widely ML techniques are used for critical decisions in our lives, the more important it becomes to hedge against potential complaints, and to have ways of redressing them. Our work takes a step in the direction of making ML methods more reliable in applications of socioeconomic importance. Of course, the downside to our methods is that they involve randomization, which might not be practical in some situations (as discussed in the previous section).

==> greedy.tex <==
\section{{\Greedy} Classifier}\label{sec:greedy}

The next question to consider is whether there is a simpler classifier that achieves similar guarantees to those given by the {\PF} classifier. We answer this question in the affirmative by presenting the iterative {\Greedy} algorithm (\cref{alg:greedy}): select the classifier that classifies the most number of data points correctly, allocate it a weight proportional to this number, discard the data points that it classifies correctly, and simply repeat the above procedure until there are no data points left. The randomized classifier {\Greedy} is defined by giving to each of these classifiers a probability proportional to its weight, i.e., the number of data points classified correctly in the corresponding iteration.

 We now show that the {\Greedy} algorithm provides a constant-factor approximation to the guarantee provided by the {\PF} classifier. Note that the first step in the \emph{while} loop of {\Greedy} (Algorithm \ref{alg:greedy}) involves using the {\ERM} agnostic learning black box. 
\begin{restatable}{theorem}{greedy}
\label{thm:greedy}
If $h_{\G}$ is the {\Greedy} classifier, then for any subset $\mathcal{S} \subseteq \mathcal{N}$ that admits a perfect classifier $h_j \in \mathcal{H}$, we have $u_S(h_{\G}) \ge \frac{\alpha}{2} + \frac{1}{2 \alpha} \left(\max\left(0, 2\alpha - 1 \right) \right)^2  \ge \frac{\alpha}{2}$, where $\frac{|S|}{n} = \alpha$.
\end{restatable}



\begin{figure}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
   \caption{{\Greedy} Classifier}
   \label{alg:greedy}
\begin{algorithmic}
    \STATE {\bfseries Input:} data set $\mathcal{N}$, family of classifiers  $\mathcal{H}$
    \STATE Initialize: $r \gets 1$, $\mathcal{S}_r \gets \mathcal{N}$
    \WHILE{$|\mathcal{S}_r| > 0$}
        \STATE $h^*_r \gets \mbox{argmax}_{h_j} u_{\mathcal{S}_r}(h_j)$
        \STATE $\mathcal{T}_r \gets \{i \in \mathcal{S}_r \mid u_i(h^*_r) = 1 \}$
        \STATE $p_r \gets \frac{|\mathcal{T}_r|}{n}$
        \STATE $\mathcal{S}_{r+1} \gets \mathcal{S}_r \setminus \mathcal{T}_r$
        \STATE $r \gets r+1$
    \ENDWHILE
    
    \STATE {\bfseries Return:} classifier $h_{\G}$ that chooses $h_s^* \in \mathcal{H}$ with probability $p_s$ for $s = 1,2,\ldots,r-1$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}  

Therefore, for any set $\mathcal{S}$ that has a perfect classifier, the average utility of {\Greedy} is at least half the average utility of Proportional Fairness; for large sets, the approximation factor is better, and approaches $1$ as $\alpha \rightarrow 1$. We complement our $\frac{\alpha}{2}$ analysis with Example 3 (in the Supplement) which shows that the above bound is tight when $\alpha \to 0$.

\paragraph{Robustness and the {\Greedy}$_k$ Algorithm}
Imagine a data set, a certain fraction of which has been corrupted with (adversarial) noise. In this case, we can use our algorithms, developed for the fairness setting, to give performance guarantees for robustness as well. Assume that the uncorrupted part of the data set is large (in terms of its fractional size), and moreover, can be classified perfectly. Let $S$ denote the uncorrupted part that admits a perfect classifier, and its size is $\alpha n$, where $\alpha \approx 1$, so that $\delta = 1 - \alpha \approx 0$. In order to measure the effect of the corrupted data, and make fine-grained distinctions between different algorithms in this regard, we focus on the loss of a classifier $h$ on subset $\mathcal{S}$, which can be defined as $\ell_\mathcal{S}(h) = 1 - u_\mathcal{S}(h)$. Therefore, if $\mathcal{S}$ has a perfect classifier $h_j$, then $\ell_\mathcal{S}(h_j) = 0$. Let $h_{\PF}$ denote the {\PF} classifier, and let $h_{\G}$ denote the {\Greedy} classifier.

\begin{restatable}{corollary}{pfgreedyloss}
\label{cor:pfgreedyloss}
For any $\delta \in (0,1/2)$, for any set $\mathcal{S}$ of size $(1-\delta)n$ that admits a perfect classifier, we have: 
$$\ell_\mathcal{S}(h_{\PF}) \le \delta; \qquad \ell_\mathcal{S}(h_{\G}) \le 2 \delta.$$
\end{restatable}

In Corollary~\ref{cor:pfgreedyloss}, the bound for {\PF} is tight because of Theorem~\ref{thm:lowerbound}, and that for {\Greedy} is tight when $\delta \to 0$ by Example 4 (in the Supplement). It is important to note that Corollary \ref{cor:pfgreedyloss} should be looked at together with  Theorems \ref{thm:pf} and \ref{thm:greedy}. In other words, taken together they imply that both {\PF} and {\Greedy} achieve fairness guarantees while still being resistant to corruption. One could ask if a different trade-off between fairness and robustness is possible, more precisely, a weaker guarantee of fairness coupled with stronger resistance to corruption. To this end, we devise a family of greedy algorithms, {\Greedy}$_k$, that interpolate between {\Greedy} and {\ERM} with 0-1 loss. We defer an exact description of {\Greedy}$_k$ and results thereof to the Supplement.

==> overview.tex <==
\subsection{Our Contributions}

\begin{enumerate}
    \item {\PF} and {\Greedy}
    \item $\delta, \gamma$-\Fair($\mathcal{G}$) and algorithm for linear case.
    \item experiments: \begin{enumerate*}
        \item {\PF} actually does better than lower bound
        \item But {\PF} guards against all kinds of sets, cannot discriminate.
        \item How does $\delta, \gamma$-\Fair($\mathcal{G}$) perform?
    \end{enumerate*}
\end{enumerate}

% We study the general multi-class classification problem. Drawing on the idea of proportional fairness from the literature on the allocation of public goods and network resources \cite{kelly1998rate, foley1970lindahl}, we come up with novel (randomized) classification methods that are:

% \begin{quote}
%     \emph{Fair for all}: providing a fairness guarantee for all possible groups simultaneously. 
% \end{quote}

% %Consequently, our methods are \emph{robust against even adversarially chosen groups}. For the average utility of any demographic group, our classifiers provide a guarantee which depends on the size of the group, as well as how hard it is to classify by itself. Therefore, even an adversary cannot add artificial demographic groups that are intrinsically hard to classify to unduly damage the performance of the classifier on all other groups. As mentioned earlier, we focus on randomized algorithms, since no deterministic classifier can hope to guard against groups defined in an adversarial fashion.

% We present the {\bf{\textsc{Proportional Fairness}}} ({\bf{\textsc{PF}}}) classifier, and show that it achieves strong theoretical guarantees for all possible groups. More precisely, we show (Theorem \ref{thm:pf}) that for any group $\mathcal{S}$ perfectly classifiable by itself, the {\PF} classifier gives a guarantee on its classification accuracy equal to the fractional size of $\mathcal{S}$, where the fractional size of a set is its size over the size of all data. In that sense, it is ``proportionally fair'', where the proportionality is with respect to the relative size of the group. We also show via a lower bound (Theorem \ref{thm:lowerbound}), that the above guarantee is the best we can hope to achieve without assumptions on the data set or the family of classifiers. No other classifier can achieve better guarantees for all groups simultaneously.

% Assuming black-box access to an agnostic learning oracle, the {\PF} classifier can be computed using a primal dual style algorithm (details are in the Supplement). Therefore, as an attractive alternative, we define the {\bf{\textsc{Greedy}}} classifier, which is conceptually simple and provides good theoretical guarantees as well. In fact, it provides a $2$-approximation to the guarantees provided by the {\PF} classifier (Theorem \ref{thm:greedy}). {\Greedy} is also much simpler to compute (again assuming black-box access to an agnostic learning oracle) since it only involves repeated calls to a $0$-$1$ loss minimizer.  

% We also delve into some consequences of our results pertaining to the {\Greedy} classifier. In particular, we show that the {\Greedy} classifier is robust in the following sense: its fairness guarantees hold even in the face of adversarial corruption of some of the data. We describe generalizations of {\Greedy} (a parametrized family of algorithms \textbf{\textsc{Greedy}$_k$}, details are in the Supplement) that are able to achieve a gradation of trade-offs between fairness and robustness to adversarial corruption.

% In addition, we evaluate the performance of our methods on real-world datasets by comparing them, on different cuts of the data, with {\ERM} methods such as Logistic Regression and AdaBoost. In particular, we see that:
% \begin{inparaenum}[(1)]
%     \item {\PF} does consistently better than the worst-case lower bound which is proportionally weaker for smaller subsets.
%     \item On subsets which the ERM methods fail to classify well, {\PF} (also {\Greedy}) does better than them, albeit at the cost of overall accuracy.
%     \item {\ERM} methods fail to do well on subsets that {\PF} finds toughest to classify.
% \end{inparaenum}

% Our theoretical and empirical results demonstrate that our fairness guarantees cannot simply be achieved by dividing the data into a set of predefined groups and running separate {\ERM}-based methods on these groups, since such an approach will not address ``hidden'' subgroups within the data, or groups that are defined orthogonal to the predefined groups. We view this as our main methodological contribution to the canon of fairness in machine learning.


% The paper is organized as follows: In \cref{sec:model}, we formally define the model and requisite notation. In \cref{sec:pf}, we describe the {\PF} classifier and the results pertaining to it. Section \ref{sec:greedy} describes {\Greedy} and its robustness properties, deferring a discussion of {\Greedy}$_k$ to the Supplement. We then discuss experimental observations in \cref{sec:experiments} and conclude the paper in \cref{sec:conclusions}. For want of space, all our proofs are provided in the Supplement.

==> pf arxiv/abstract.tex <==
% Existing group-based notions of fairness in classification, such as \emph{statistical parity} and \emph{equality of opportunity}, are defined by comparing statistical measures of performance across different groups (based on race, gender, etc.) in the data. In such approaches, the goal is to achieve the same performance on all groups that are specified beforehand. Consequently, no guarantees are provided for communities that the algorithm designer did not foresee; and a group that is inherently harder to classify may hold back the performance on all other groups.

% We first devise the {\sc\texttt{Proportional Fairness}} ({\PF}) classifier which provides a fairness guarantee for all groups simultaneously: for any group $S$, the accuracy on $S$ is guaranteed to be at least that of the optimal classifier for $S$, scaled by the relative size of $S$ in the data set. However, since {\PF} guards against all possible groups, some of which could be too complex to be relevant, its worst-case theoretical guarantees are proportionally weaker for smaller subsets. 

% To this end, we present a more streamlined notion of fairness - $\gamma,\delta$-\Fair$(\mathcal{G})$ - which for any group $g$ in the class $\mathcal{G}$, seeks to achieve a performance within a multiplicative factor $\delta$ and an additive factor $\gamma$ of that of the optimal classifier on $g$. Aiming for such a guarantee, one which does not depend on the size of $g$, results in a non-convex problem, and we design novel techniques to get around this difficulty when $\mathcal{G}$ is the set of linear hypotheses. We show that our algorithms work well on real-world data sets, and present interesting comparative insights on their performance.


Standard approaches to group-based notions of fairness, such as \emph{parity} and \emph{equalized odds}, try to equalize absolute measures of performance across known groups (based on race, gender, etc.). Consequently, a group that is inherently harder to classify may hold back the performance on other groups; and no guarantees can be provided for unforeseen groups. Instead, we propose a fairness notion whose guarantee, on each group $g$ in a class $\mathcal{G}$, is relative to the performance of the best classifier on $g$. We apply this notion to broad classes of groups, in particular, where (a) $\mathcal{G}$ consists of all possible groups (subsets) in the data, and (b) $\mathcal{G}$ is more streamlined.

For the first setting, which is akin to groups being completely unknown, we devise the {\sc PF} (Proportional Fairness) classifier, which guarantees, on any possible group $g$, an accuracy that is proportional to that of the optimal classifier for $g$, scaled by the relative size of $g$ in the data set. Due to including all possible groups, some of which could be too complex to be relevant, the worst-case theoretical guarantees here have to be proportionally weaker for smaller subsets.

For the second setting, we devise the  {\sc BeFair} (Best-effort Fair) framework which seeks an accuracy, on every $g \in \mathcal{G}$, which approximates that of the optimal classifier on $g$, independent of the size of $g$. Aiming for such a guarantee results in a non-convex problem, and we design novel techniques to get around this difficulty when $\mathcal{G}$ is the set of linear hypotheses. We test our algorithms on real-world data sets, and present interesting comparative insights on their performance.


==> pf arxiv/broader_impact.tex <==
\section*{Broader Impact}
The classification methods presented in this paper are geared towards guaranteeing fairness to all possible groups in the data. Such methods are extremely useful in situations where it is unclear what the protected groups should be. In other cases, when we try to optimize for a certain notion of fairness for some pre-defined groups, questions can be raised about the performance achieved on a group not accounted for beforehand, and thereby lead to complaints from such groups. Our methods can also serve as a baseline to make sure that there is no potential group being unduly affected. The more widely ML techniques are used for critical decisions in our lives, the more important it becomes to hedge against potential complaints, and to have ways of redressing them. Our work takes a step in the direction of making ML methods more reliable in applications of socioeconomic importance. Of course, the downside to our methods is that they involve randomization, which might not be practical in some situations (as discussed in the previous section).

==> pf arxiv/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
In this paper, we study group fairness in the (multi-class) classification setting. We propose a notion based on best-effort guarantees, which requires each group in a class $\mathcal{G}$ to have a classification accuracy that is as close as possible to the optimal for that group. When $\mathcal{G}$ consists of all possible groups, we show that {\PF} achieves the theoretical optimum in our setting. When $\mathcal{G}$ consists of linearly separable groups, we can do much better via the {\BeFair} algorithm, which crucially depends on convexification techniques to solve an essentially non-convex problem. We also test our methods on real-world datasets and show that they perform well in practice, especially the {\BeFair} method.

% Some questions follow directly as possible future directions. Are there other easy-to-compute classifiers that give a better approximation to the guarantees of {\PF}? Note that for $k=1$, {\Greedy}$_k$ can be thought of as proportional fairness as limited to the successive marginal gains given by the classifiers in Algorithm \ref{alg:greedy}, and as $k \to \infty$ we get the standard {\ERM} classifier with $0$-$1$ loss. Are there other families of classifiers that can thread a different trade-off than that of {\Greedy}$_k$?

One interesting question for future work is to extend our techniques for more involved classes of groups, say, for example, when $\mathcal{G}$ consists of all groups that can be identified by a fixed neural network. Similar extensions of the hypothesis space $\mathcal{H}$ are also worth looking at. Moreover, in some applications (bail/loan decisions, college admissions, etc.), false negatives and false positives play drastically different roles. Can our framework be extended to deal with such considerations? Can it also be extended to multi-class classification? Note that the guarantees of {\PF} carry over to this setting directly. We would also like to point out that randomized classifiers are not always desirable and have some limitations in practice \citep{cotter2019making}. How to think about best-effort fairness of deterministic classifiers with unknown groups is another interesting open question.


==> pf arxiv/experiments.tex <==
\section{Experiments}\label{sec:experiments}

%  The primary goal of our experiments is to show how our algorithm is able to find good solutions to Problem \ref{prob:dGPF} for small values of $\delta$ and $\gamma$. We will also show how, in practice, the performance of {\PF} is significantly better than what is suggested by the worst-case lower bound via \cref{thm:pf} (which is proportionally weaker for smaller subsets). However, {\PF} is constrained to factor in all possible groups in the data (some possibly unnecessarily complex), and therefore takes a larger hit in performance. 

 The primary goal of our experiments is to show that the {\BeFair} algorithm works extremely well in practice. As we discuss below, {\BeFair} achieves its intended purpose (as discussed in the previous section), by achieving strong best-effort fairness guarantees uniformly over all linearly separable groups. In particular, it is able to achieve a performance that is a close approximation of the best possible on these groups (as given in Problem \ref{prob:dGPF}) for small values of $\delta$ and $\gamma$. In addition, we will also evaluate the {\PF} algorithm and show how it behaves differently from {\BeFair}, on account on having to provide guarantees for all possible groups, even those corresponding to a high VC dimension.  We also show how, in practice, the performance of {\PF} seems to be better than what is suggested by the worst-case lower bound via \cref{thm:pf} (which is proportionally weaker for smaller groups).

We work with two data sets: \texttt{adult}, the Adult\footnote{\tiny 48842 instances, 14 features, \url{https://archive.ics.uci.edu/ml/datasets/Adult}} dataset from the UCI Machine Learning Repository, and \texttt{compas}, the COMPAS\footnote{\tiny 6172 instances, 8 features, \url{https://www.propublica.org/article/how-we-analyzed-the-compas-recidivism-algorithm}} Risk of Recidivism data set \citep{angwin2016machine}. Both have binary labels and a mixture of numerical and categorical features. Using these data sets, we compare and contrast the following 
methods (recalling their definitions from earlier):
\begin{enumerate}
    \item {\PF}: As the exact solution of {\PF} is computationally inefficient, we use {\hPF}, a heuristic (details in the Appendix) inspired by Reweighted Approval Voting. \citep{aziz2017justified}. In what follows, we refer to {\hPF} as {\PF}. 
    \item {$\delta$-\BeFair} as described in Section \ref{sec:pf_error}.
    \item {\ERM} methods: We use {\LR} (Logisitic Regression), since it performs best here. We also compare overall accuracy with {\Ada} (AdaBoost), an ensemble method.
    \item The lower bound given by \cref{cor:pf}.
\end{enumerate}


\begin{table}
\small
\setlength\tabcolsep{4pt}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    &\LR &\Ada & \hPF & $1.0$-\BeFair & $1.1$-\BeFair\\ \hline
    \texttt{adult} & 0.83 & 0.84 & 0.78 & 0.79 & 0.80 \\ \hline
     \texttt{compas} & 0.75 & 0.75 & 0.64 & 0.70 & 0.71 \\ \hline
\end{tabular}
\caption{Overall test accuracy of various methods.}
\label{tab:overall}
\end{table}

In \cref{tab:overall}, we present the overall accuracy of various methods, i.e., that measured on the entire test set. As there is a trade-off between ensuring fairness for groups and maximizing overall accuracy, {\PF} has a lower overall accuracy compared to other methods. $\delta$-{\BeFair} is much closer to the ERM baselines (especially as seen on the \texttt{compas} dataset, even for a small value of $\delta = 1.1$. Larger values of $\delta$ can only increase accuracy as the fairness constraints become laxer.

\subsection{Evaluating the performance of  {\BeFair}}\label{sec:pfvsbefair}

We first define Maximum Additive Error ($\mae_\delta$), parametrized by $\delta$, of any given classifier $h$.
\begin{definition}[$\mae_\delta(h)$]\label{def:maedelh}
For a given $h$, and $\delta$, 
$\mae_\delta(h) = \max_{g \in \mathcal{G}}\err_g(h) - \delta \cdot \err_g(h^*_g) $.
\end{definition}
For a given $h$, $\mae_\delta(h)$ specifies, for the worst-off group $g$, how much difference there is between the error of $h$ and that of the best classifier for $g$ scaled by $\delta$. 

For instance, $\mae_\delta(\textsc{BeFair})$ can be computed by searching over different values of $\gamma$ to pick the smallest that gives a feasible solution for the $\delta$-\BeFair($\gamma$) problem. On the other hand, $\mae_\delta(\textsc{ERM})$ can be computed by solving the Adversary's problem (Equation \ref{eqn:advobj} modified as per $\delta$) for $h = \ERM$. 

In Figure \ref{fig:alpha_vs_beta}, we compare $\mae_\delta$ of {\ERM} and {\BeFair} for $\delta = 1.0,1.05, \ldots, 1.30$. Errors are reported as a percentage of the entire data set.

% Another quantity of interest is the following:
% \begin{definition}[$\beta_\delta$] \label{def:delbeta}
% For a given $\delta$, 
% $\beta_\delta$ is the minimum value of $\gamma$ for which Problem \ref{prob:dGPF} is feasible.
% \end{definition}
% Defined this way, $\beta_\delta$ is a measure of how close the randomized classifier obtained via our algorithm is to achieving, for all groups $g \in \mathcal{G}$, an error of at most $\delta$ times that of the minimum error on $g$ (over $h \in \mathcal{H}$).

% We will use $\delta$-{\BeFair} to refer to the solution obtained via the method proposed in this section as follows:

% \begin{definition}[$\delta$-{\BeFair}] \label{def:delbefair}
% For a given $\delta$, 
% $\delta$-{\BeFair} is the solution to the $\delta$-{\BeFair}($\beta_\delta$) problem.
% \end{definition}

% Recall the definitions of $\alpha(\delta)$ and $\beta(\delta)$ from Section \ref{sec:pf_error}: $\alpha_\delta$ is the minimum value of $\gamma$ for which ERM ({\LR}) achieves a $\delta$ best-effort guarantee. $\beta(\delta)$ is the minimum value of $\gamma$ for which {\BeFair} achieves a $\delta$ best-effort guarantee. By using $\alpha(\delta)$ and $\beta(\delta)$, we are effectively comparing how much extra error is accrued by {\ERM} and {\BeFair}, respectively, to achieve a $\delta$ best-effort guarantee.
\begin{figure}[ht]\centering
\begin{subfigure}{0.44\linewidth}\centering
\includegraphics[scale=0.26]{final_compas_alpha_vs_beta.png}
\end{subfigure}%
\quad
\begin{subfigure}{0.44\linewidth}\centering
\includegraphics[scale=0.26]{final_adult_alpha_vs_beta.png}
\end{subfigure}
\caption{Comparing $\mae_\delta$ between {\ERM} and {\BeFair} for varying values of $\delta$.}
\label{fig:alpha_vs_beta}
\end{figure}

Many key observations can be made from this plot: 
\begin{enumerate}[label = (\alph*)]
    \item As we increase $\delta$, the $\mae_\delta$ of both {\ERM} and {\BeFair} decrease. This is because the best-effort constraints get laxer with increasing $\delta$.
    \item Even for $\delta = 1.0$, {\BeFair} achieves an improvement  over {\ERM} of close to 50\% (since $\mae_\delta(\textsc{BeFair})$ is about half of $\mae_\delta(\textsc{ERM})$) on \texttt{compas}, and 33\% on \texttt{adult}, in the $\mae_\delta$ value.
    \item For a slightly larger value of $\delta = 1.10$, we get an extremely low value for $\mae_\delta(\textsc{BeFair})$ of around $1\%$, which means {\BeFair} gets a strong approximation. Therefore, {\BeFair} is able to achieve an multiplicative error of $0.1$, with an additive error of around $1$\%.
    \item $\mae_\delta(\textsc{ERM})$ decreases linearly with $\delta$, while most of the improvement in $\mae_\delta(\textsc{BeFair})$ comes from increasing $\delta$ from $1$ to $1.05$. In other words, {\BeFair} is able to extract a bigger improvement with a small increase of $\delta$.
\end{enumerate}
Overall, {\BeFair} achieves low $\mae_\delta$ for small values of $\delta = 1.05, 1.1$.



%We see that even for a relatively small value of $\delta$, say $1.05$, we are able to achieve a $\alpha$ of less than $0.015$. Maximum gain is achieved in the initial increase of $\delta$ from $1$ to $1.05$, and the gain from there onward yields marginal returns. 



\subsection{Comparison of {\PF} with {\BeFair}:}
In \Cref{fig:compas_pf_vs_fp_cum}, we order (on the $x$ axis) the data points in the test set in ascending order of their scores (i.e., confidence of predicting the true label) given by {\LR}. For each point $x$, the $y$ axis shows the accuracy of various methods on the subset consisting of all points from $0$ through $x$.
If we imagine the {\LR} scores as a measure of how easy the points are to classify correctly: then we see that {\PF} gets a more uniform error on all these sets, whereas $1.1$-{\BeFair} has lower error on sets with higher {\LR} scores. This is because the groups where {\BeFair} has high error are probably too complex to be meaningful practically. On the other hand, {\PF} must provide uniform guarantees over all groups, even those corresponding to large VC dimensions, and therefore has a uniformly higher error on them. 
\begin{figure}
    \centering
    \includegraphics[scale=0.15]{final_pf_vs_fp_edited.png}
    \caption{Error on subsets of varying sizes (\texttt{compas}): $x$ axis denotes points in ascending order of {\LR} scores. $y$ axis denotes error accrued on the subset containing points up to $x$.} 
    \label{fig:compas_pf_vs_fp_cum}
\end{figure}


\subsection{Comparison of {\PF} with the theoretical lower bound}\label{subsec:exp:lowerbound}
In \Cref{fig:compas_pf-vs-erm_cum} (left), we order (on the $x$ axis) the data points in the test set in ascending order of their scores (i.e., confidence of predicting the true label) given by {\Ada}. For each point $x$, the $y$ axis shows the accuracy of various methods on the subset consisting of all points from $0$ through $x$. \Cref{fig:compas_pf-vs-erm_cum} (right) does the same with {\PF} scores.

We see that the accuracy of {\PF} is much higher than the worst-case lower bound. {\PF} comes close to the lower bound for larger subsets, especially for those that are easy to classify (see the Appendix for more details). Note that the lower bound \emph{is not monotonic} because it depends on both the size of the subset and the best possible classification accuracy on it (\cref{cor:pf}). Also, in  \Cref{fig:compas_pf-vs-erm_cum} (right), ERM methods do worse because the points with low {\hPF} scores are inherently much harder to classify.

\begin{figure}\centering
\begin{subfigure}{0.44\linewidth}\centering
\includegraphics[scale=0.26]{final_compas_pf-vs-ada_cum.png}
\end{subfigure}%
\quad
\begin{subfigure}{0.44\linewidth}\centering
\includegraphics[scale=0.26]{final_compas_erm-vs-pf_cum.png}
\end{subfigure}
\caption{Accuracy on subsets of varying size (\texttt{compas}): $x$ axis denotes points in ascending order of {\Ada} (left) and {\hPF} (right) scores. $y$ axis denotes accuracy on the subset containing points up to $x$.}
\label{fig:compas_pf-vs-erm_cum}
\end{figure}


==> pf arxiv/greedy.tex <==
\section{{\Greedy} Classifier}\label{sec:greedy}

The next question to consider is whether there is a simpler classifier that achieves similar guarantees to those given by the {\PF} classifier. We answer this question in the affirmative by presenting the iterative {\Greedy} algorithm (\cref{alg:greedy}): select the classifier that classifies the most number of data points correctly, allocate it a weight proportional to this number, discard the data points that it classifies correctly, and simply repeat the above procedure until there are no data points left. The randomized classifier {\Greedy} is defined by giving to each of these classifiers a probability proportional to its weight, i.e., the number of data points classified correctly in the corresponding iteration.

 We now show that the {\Greedy} algorithm provides a constant-factor approximation to the guarantee provided by the {\PF} classifier. Note that the first step in the \emph{while} loop of {\Greedy} (Algorithm \ref{alg:greedy}) involves using the {\ERM} agnostic learning black box. 
\begin{restatable}{theorem}{greedy}
\label{thm:greedy}
If $h_{\G}$ is the {\Greedy} classifier, then for any subset $\mathcal{S} \subseteq \mathcal{N}$ that admits a perfect classifier $h_j \in \mathcal{H}$, we have $u_S(h_{\G}) \ge \frac{\alpha}{2} + \frac{1}{2 \alpha} \left(\max\left(0, 2\alpha - 1 \right) \right)^2  \ge \frac{\alpha}{2}$, where $\frac{|S|}{n} = \alpha$.
\end{restatable}



\begin{figure}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
   \caption{{\Greedy} Classifier}
   \label{alg:greedy}
\begin{algorithmic}
    \STATE {\bfseries Input:} data set $\mathcal{N}$, family of classifiers  $\mathcal{H}$
    \STATE Initialize: $r \gets 1$, $\mathcal{S}_r \gets \mathcal{N}$
    \WHILE{$|\mathcal{S}_r| > 0$}
        \STATE $h^*_r \gets \mbox{argmax}_{h_j} u_{\mathcal{S}_r}(h_j)$
        \STATE $\mathcal{T}_r \gets \{i \in \mathcal{S}_r \mid u_i(h^*_r) = 1 \}$
        \STATE $p_r \gets \frac{|\mathcal{T}_r|}{n}$
        \STATE $\mathcal{S}_{r+1} \gets \mathcal{S}_r \setminus \mathcal{T}_r$
        \STATE $r \gets r+1$
    \ENDWHILE
    
    \STATE {\bfseries Return:} classifier $h_{\G}$ that chooses $h_s^* \in \mathcal{H}$ with probability $p_s$ for $s = 1,2,\ldots,r-1$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}  

Therefore, for any set $\mathcal{S}$ that has a perfect classifier, the average utility of {\Greedy} is at least half the average utility of Proportional Fairness; for large sets, the approximation factor is better, and approaches $1$ as $\alpha \rightarrow 1$. We complement our $\frac{\alpha}{2}$ analysis with Example 3 (in the Supplement) which shows that the above bound is tight when $\alpha \to 0$.

\paragraph{Robustness and the {\Greedy}$_k$ Algorithm}
Imagine a data set, a certain fraction of which has been corrupted with (adversarial) noise. In this case, we can use our algorithms, developed for the fairness setting, to give performance guarantees for robustness as well. Assume that the uncorrupted part of the data set is large (in terms of its fractional size), and moreover, can be classified perfectly. Let $S$ denote the uncorrupted part that admits a perfect classifier, and its size is $\alpha n$, where $\alpha \approx 1$, so that $\delta = 1 - \alpha \approx 0$. In order to measure the effect of the corrupted data, and make fine-grained distinctions between different algorithms in this regard, we focus on the loss of a classifier $h$ on subset $\mathcal{S}$, which can be defined as $\ell_\mathcal{S}(h) = 1 - u_\mathcal{S}(h)$. Therefore, if $\mathcal{S}$ has a perfect classifier $h_j$, then $\ell_\mathcal{S}(h_j) = 0$. Let $h_{\PF}$ denote the {\PF} classifier, and let $h_{\G}$ denote the {\Greedy} classifier.

\begin{restatable}{corollary}{pfgreedyloss}
\label{cor:pfgreedyloss}
For any $\delta \in (0,1/2)$, for any set $\mathcal{S}$ of size $(1-\delta)n$ that admits a perfect classifier, we have: 
$$\ell_\mathcal{S}(h_{\PF}) \le \delta; \qquad \ell_\mathcal{S}(h_{\G}) \le 2 \delta.$$
\end{restatable}

In Corollary~\ref{cor:pfgreedyloss}, the bound for {\PF} is tight because of Theorem~\ref{thm:lowerbound}, and that for {\Greedy} is tight when $\delta \to 0$ by Example 4 (in the Supplement). It is important to note that Corollary \ref{cor:pfgreedyloss} should be looked at together with  Theorems \ref{thm:pf} and \ref{thm:greedy}. In other words, taken together they imply that both {\PF} and {\Greedy} achieve fairness guarantees while still being resistant to corruption. One could ask if a different trade-off between fairness and robustness is possible, more precisely, a weaker guarantee of fairness coupled with stronger resistance to corruption. To this end, we devise a family of greedy algorithms, {\Greedy}$_k$, that interpolate between {\Greedy} and {\ERM} with 0-1 loss. We defer an exact description of {\Greedy}$_k$ and results thereof to the Supplement.

==> pf arxiv/intro.tex <==
\section{Introduction}\label{sec:intro}
%As machine learning plays a bigger role in applications that have a significant impact on people's lives (including criminal justice~\citep{}, lending~\citep{}, and so on), it is important to have models that are fair.

%Existing fairness approaches typically fix a list of demographic groups, and then ask for (approximate) equality of some statistical measure across these groups.  One popular approach is to ask for equal false positive or negative rates, or the same number of false positive or negative points in each group (see, e.g.,~\citep{KearnsNRW18, HossainMS19}).

%One major problem with many existing fairness notions is that they are not robust to the error in the demographic groups. There are two types of error that could appear in the list of demographics: 1) Missing demographics: a group of people that we want to protect and be fair to, which is not listed in the input demographics.2) Adversarial demographics: an arbitrary group of people that is put together by the adversary as a ``fake'' demographic group to hurt the algorithm's performance on other groups.

Machine learning is playing an ever-increasing role in making decisions that have a significant impact on our lives. Of late, we have seen the deployment of machine learning methods to provide advice for decisions pertaining to criminal justice \citep{angwin2016machine, berk2018fairness}, credit/lending  \citep{koren2016does}, health/medicine \citep{rajkomar2018ensuring}, etc. Given the concerns of disparate impact and bias in this regard \citep{angwin2016machine, barocas2016big}, it is imperative that machine learning models are fair.

The question of defining notions of fairness, and developing methods to achieve them, has received a great deal of attention \citep{barocas2017fairness, binns2017fairness}. A common theme among the many approaches proposed thus far \citep{kleinberg2018inherent, chouldechova2017fair} is to fix beforehand a list of protected groups, and then ask for the (approximate) equality of some statistical measure across them. For example, \emph{parity} seeks to equalize the accuracy across the given groups \citep{calders2009building}, while \emph{equalized odds} seeks to equalize false positive or false negative rates \citep{hardt2016equality}.

Classical definitions of fairness from microeconomics have also found application in machine learning \citep{balcan2019envy, chen2019proportionally, HossainMS19}. In particular, there has been recent work \citep{zafar2017parity, ustun2019fairness} on adapting the notion of \emph{envy-freeness}, which is born out of fair division theory \citep{brams1996fair}, to a group-based variant tailored to (binary) classification -- every given pre-defined group should prefer the way it is classified (on aggregate) in comparison to how it would have been if it assumed the identity of some other group. 

A major drawback of the aforementioned approaches is that they aim for an absolute guarantee: when some of the groups are inherently harder to classify than others, trying to achieve a particular measure of fairness, say equalized odds \citep{hardt2016equality}, could do more harm than good by bringing down the accuracy on a group that is easier to classify (see Figure \ref{fig:harm} for an example). In this paper, we take a more relative \emph{best-effort} approach: aiming for guarantees that are defined in terms of how well each group can be classified in itself.

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{harm_example.png}
  %\hspace{0.10\textwidth}
    \caption{Given two groups Blue and Yellow (with true labels as shown), we have to choose just between the two classifiers $x=0$ and $y=0$. The Blue group is inherently harder to classify. Equalized odds makes us choose the classifier $x=0$, thereby hurting the Yellow group. We could choose $y=0$ with no aggregate effect on Blue, doing much better on Yellow. 
    } 
    \label{fig:harm}
\end{figure}

Another drawback of the standard approaches to fairness is that they depend critically on the specification of groups (via sensitive features such as race, gender, etc.). In many cases, the sensitive features are either missing \citep{chen2019fairness}, or unusable, considering the need to adhere to \emph{treatment parity} and anti-discrimination laws \citep{barocas2016big}. Even if they can be used, it is sometimes not clear what the right categorization within them should be. For instance, it could be that a particular demographic group, which is defined on the basis of a shared cultural or ethnic feature, is actually a collection of hidden subgroups that are otherwise quite heterogeneous in terms of other socio-economic indicators \citep{meier2012latino, chang2011debunking}. %noire2011fair}. 
Therefore, mis-specifying or mis-calibrating the protected groups could end up hurting some groups within the data, potentially leading to unintended consequences such as a feeling of resentment among them \citep{hoggett2013fairness}.


% One major drawback of the aforementioned approaches is that they depend critically on the specification of protected groups (based on sensitive attributes such as race, gender, or combinations thereof). In many cases, the sensitive features are either missing \citep{chen2019fairness}, or cannot be used considering the need to adhere to \emph{treatment parity} and anti-discrimination laws \citep{barocas2016big}. Even if they could be used, it is sometimes not clear what the right categorization within them should be. For instance, it could be that a particular demographic group, which is defined on the basis of a shared cultural or ethnic feature, is actually a collection of hidden subgroups that are otherwise quite heterogeneous in terms of general socio-economic indicators \citep{meier2012latino, chang2011debunking, noire2011fair}. Therefore, if the protected groups are mis-specified or mis-calibrated, it could end up hurting some groups within the data, potentially leading to unintended consequences such as a feeling of resentment among them \citep{hoggett2013fairness}.


%not resilient to mis-specifications in the list of demographic groups, which could be of three types: \begin{inparaenum}[(a)]
%\item missing demographics: a group of people that we want to protect and be fair to, but is not listed in the demographics input;
%\item adversarial demographics: a group that is put together by an adversary as a ``fake'' demographic group to hurt the algorithm's performance on other groups;
%\item hindsight demographics: a group that is defined ex-post as evidence as to why the algorithm is unfair.
%\end{inparaenum}

We  use  the  following  instructive  albeit  stylized  example to illustrate the effect of missing group information.
\begin{example}
As shown below in Table \ref{tab:example1}, there are two binary features $a,b \in \{0,1\}$, and a hidden demographic feature $c \in \{0,1\}$. The target label $y$ follows the formula $y = (a \wedge c) \vee (b \wedge \neg c)$: if the hidden feature $c = 1$, then $a$ is a perfect classifier, and if $c=0$, then $b$ is a perfect classifier. For brevity, we define three groups: $P = \{(1,0,0), (0,1,0)\}$, $Q = \{(1,0,1), (0,1,1)\}$, and $R = (P \cup Q)^\mathsf{c}$.

As a concrete example, suppose each data point corresponds to a job candidate.
The hidden feature $c$ corresponds to \emph{gender}, $(a,b)$ correspond to measures of two different traits, and $y$ the assignment to one of two jobs. Suppose the family of available classifiers is $\mathcal{H} = \{a,b\}$. It can be seen that any of these classifiers does poorly in terms of fairness for groups based on the hidden feature $c$. 

Consider the classifier $a$ (in this case, a solution to the standard {Empirical Risk Minimization} ({\ERM}) with $0$-$1$ loss), which correctly classifies all data except those in $P$. Therefore, the {\ERM} classifier $a$ is unfair to those of gender $0$. Our {\PF} classifier (which we shall see later) gets around this issue by randomizing between $a$ and $b$. This allows us to classify $P$ and $Q$ correctly with probability $0.5$, and $R$ correctly with probability $1$. Note that the {\PF} classifier is able to treat every gender equally in expectation, even without access to the gender labels.
\end{example}

\begin{table}
\small
\centering
\begin{tabular}{c|cccccccc}
 $a$ & $1$&  $1$&  $0$&  $0$&  $1$&  $1$&  $0$&  $0$\\ 
 $b$ & $1$&  $0$&  $1$&  $0$&  $1$&  $0$&  $1$&  $0$\\
 $c$ & $1$&  $1$&  $1$&  $1$&  $0$&  $0$&  $0$&  $0$\\\hline
 $y$ & $1$&  $1$&  $0$&  $0$&  $1$&  $0$&  $1$&  $0$
 \smallskip
\end{tabular}
\caption{$a,b$ are visible features, $c$ is a hidden ``demographic'' feature, and $y$ is the target label.}
\label{tab:example1}
\end{table}

In order to deal with the above issues, we take a best-effort approach to fairness, one that can be applied to broad classes of groups. If the group identities were well defined and limited in number, simple solutions work: for example, one could perhaps train decoupled classifiers \citep{ustun2019fairness, dwork2018decoupled}. With the unavailability or mis-specification of group information, however, the problem is much more interesting. In this regard, we look at two settings -- where the groups taken into account are given by \begin{enumerate*}[label=(\alph*)]
    \item all possible subsets in the data, and
    \item a more streamlined class of groups, such as all linearly separable ones. 
\end{enumerate*}

In the former setting, we are effectively reasoning about fairness even though there are no pre-specified groups. Standard statistical notions are of no use in this regard, for, as noted by \citet{KearnsNRW18}, ``we cannot insist on any notion of statistical fairness for every subgroup of the population: for example, any imperfect classifier could be accused of being unfair to the subgroup of individuals defined ex-post as the set of individuals it mis-classified.''

In fact, such a limitation also applies to any deterministic classifier. Therefore, focusing on randomized classifiers, the questions we consider first (Section \ref{sec:pf}) are: \emph{What is the best possible best-effort guarantee that can be achieved for all groups simultaneously?} We will see that, on account of taking all groups into account, some of which could be too complex to be meaningful in practice, we have to settle for guarantees that are proportionally weaker for smaller subsets. \emph{Are there algorithms that achieve such a guarantee?} We answer this question in the affirmative by devising the Proportional Fairness (\PF) classifier.

The next natural question is: \emph{can we do better if we consider a more streamlined class of groups?} We will see (Section \ref{sec:pf_error}) that this is indeed the case. We note here that standard fairness notions (such as \emph{parity}) can also be applied in such settings, by effectively solving a convex optimization problem \citep{KearnsNRW18}. In our best-effort fairness (\BeFair) approach, even when we consider linearly separable groups, we need to solve a non-convex problem. A major contribution of our work is devising a way of dealing with this difficulty, and at that, one that works well in practice. In Section \ref{sec:experiments}, we \emph{evaluate all our algorithms on real-world datasets}. We see that our {\BeFair } approach is able to achieve strong best-effort guarantees, significantly better than standard {\ERM } classifiers. We also present several empirical insights on the performance on {\PF}, mostly in line with our theoretical results.

A more detailed overview of our results are provided in Section \ref{sec:model}. All our proofs are provided in the Appendix.

% These considerations lead us to the following questions:
% \begin{itemize}
%     \item Allowing for randomized classifiers, is there a systematic way of defining fairness, even for multi-class classification? Are there algorithms that work for such a definition of fairness?
%     \item What are the limitations of such an approach, especially given that all possible groups are taken into consideration?
%     \item Can we do better if we somehow limit the classes of groups considered, perhaps those of a finite VC dimension?
%     \item How does such an approach work on real-world data sets?
% \end{itemize}
% The goal of this paper is to answer these questions, as we discuss next.

==> pf arxiv/overview.tex <==
\subsection{Our Contributions}

\begin{enumerate}
    \item {\PF} and {\Greedy}
    \item $\delta, \gamma$-\Fair($\mathcal{G}$) and algorithm for linear case.
    \item experiments: \begin{enumerate*}
        \item {\PF} actually does better than lower bound
        \item But {\PF} guards against all kinds of sets, cannot discriminate.
        \item How does $\delta, \gamma$-\Fair($\mathcal{G}$) perform?
    \end{enumerate*}
\end{enumerate}

% We study the general multi-class classification problem. Drawing on the idea of proportional fairness from the literature on the allocation of public goods and network resources \cite{kelly1998rate, foley1970lindahl}, we come up with novel (randomized) classification methods that are:

% \begin{quote}
%     \emph{Fair for all}: providing a fairness guarantee for all possible groups simultaneously. 
% \end{quote}

% %Consequently, our methods are \emph{robust against even adversarially chosen groups}. For the average utility of any demographic group, our classifiers provide a guarantee which depends on the size of the group, as well as how hard it is to classify by itself. Therefore, even an adversary cannot add artificial demographic groups that are intrinsically hard to classify to unduly damage the performance of the classifier on all other groups. As mentioned earlier, we focus on randomized algorithms, since no deterministic classifier can hope to guard against groups defined in an adversarial fashion.

% We present the {\bf{\textsc{Proportional Fairness}}} ({\bf{\textsc{PF}}}) classifier, and show that it achieves strong theoretical guarantees for all possible groups. More precisely, we show (Theorem \ref{thm:pf}) that for any group $\mathcal{S}$ perfectly classifiable by itself, the {\PF} classifier gives a guarantee on its classification accuracy equal to the fractional size of $\mathcal{S}$, where the fractional size of a set is its size over the size of all data. In that sense, it is ``proportionally fair'', where the proportionality is with respect to the relative size of the group. We also show via a lower bound (Theorem \ref{thm:lowerbound}), that the above guarantee is the best we can hope to achieve without assumptions on the data set or the family of classifiers. No other classifier can achieve better guarantees for all groups simultaneously.

% Assuming black-box access to an agnostic learning oracle, the {\PF} classifier can be computed using a primal dual style algorithm (details are in the Supplement). Therefore, as an attractive alternative, we define the {\bf{\textsc{Greedy}}} classifier, which is conceptually simple and provides good theoretical guarantees as well. In fact, it provides a $2$-approximation to the guarantees provided by the {\PF} classifier (Theorem \ref{thm:greedy}). {\Greedy} is also much simpler to compute (again assuming black-box access to an agnostic learning oracle) since it only involves repeated calls to a $0$-$1$ loss minimizer.  

% We also delve into some consequences of our results pertaining to the {\Greedy} classifier. In particular, we show that the {\Greedy} classifier is robust in the following sense: its fairness guarantees hold even in the face of adversarial corruption of some of the data. We describe generalizations of {\Greedy} (a parametrized family of algorithms \textbf{\textsc{Greedy}$_k$}, details are in the Supplement) that are able to achieve a gradation of trade-offs between fairness and robustness to adversarial corruption.

% In addition, we evaluate the performance of our methods on real-world datasets by comparing them, on different cuts of the data, with {\ERM} methods such as Logistic Regression and AdaBoost. In particular, we see that:
% \begin{inparaenum}[(1)]
%     \item {\PF} does consistently better than the worst-case lower bound which is proportionally weaker for smaller subsets.
%     \item On subsets which the ERM methods fail to classify well, {\PF} (also {\Greedy}) does better than them, albeit at the cost of overall accuracy.
%     \item {\ERM} methods fail to do well on subsets that {\PF} finds toughest to classify.
% \end{inparaenum}

% Our theoretical and empirical results demonstrate that our fairness guarantees cannot simply be achieved by dividing the data into a set of predefined groups and running separate {\ERM}-based methods on these groups, since such an approach will not address ``hidden'' subgroups within the data, or groups that are defined orthogonal to the predefined groups. We view this as our main methodological contribution to the canon of fairness in machine learning.


% The paper is organized as follows: In \cref{sec:model}, we formally define the model and requisite notation. In \cref{sec:pf}, we describe the {\PF} classifier and the results pertaining to it. Section \ref{sec:greedy} describes {\Greedy} and its robustness properties, deferring a discussion of {\Greedy}$_k$ to the Supplement. We then discuss experimental observations in \cref{sec:experiments} and conclude the paper in \cref{sec:conclusions}. For want of space, all our proofs are provided in the Supplement.

==> pf arxiv/pf.tex <==
\section{Best-effort guarantee for all groups}\label{sec:pf}
The first question to ask is whether there is a fundamental limit on how well one can hope to do with respect to fairness in the setting where $\mathcal{G} = 2^\mathcal{N}$. Since we are dealing with a notion of fairness that is measured relative to the family of classifiers at hand, we first want to understand what the best guarantee that can be given is (in the form of a worst-case bound), with no conditions on the type of classifiers used. 

\begin{restatable}{theorem}{lowerbound} \label{thm:lowerbound}
On any data set $\mathcal{N}$, there is no randomized classifier $h$ (for some $\mathcal{H}$) such that for all $g \subseteq \mathcal{N}$ admitting a perfect classifier $h^*_g \in \mathcal{H}$ (i.e., $u_g(h^*_g) = 1$), we have $u_g(h) > \frac{|g|}{|\mathcal{N}|}$.
\end{restatable}

This theorem shows that, in terms of how much utility is accrued by each of the perfectly classified sets, the best bound we can hope to target is one proportional to the fractional size of the given set of data points. Note that for every instance, there exists some $\mathcal{H}$, such that the claim of the theorem holds -- this is not true more generally in the sense that there could exist some $\mathcal{H}$ for which the claim does not hold as shown by Example 2 (in the Appendix).

\subsection{Proportional Fairness ({\PF}) Classifier}
We now demonstrate a classifier that matches the above bound as long as the utilities $u_i(h_j)$'s are binary (which holds in our model, but could also be encountered in other scenarios involving resource allocation discussed in \cref{sec:related}); as mentioned before, this captures multi-class classification as well. The Proportional Fairness classifier is defined as follows:

\begin{definition}[Proportional Fairness ({\PF})]
\label{def:pf}
Given an instance $(\mathcal{N}, \mathcal{H})$, the {\PF} classifier $h_{\PF}$ is the one that maximizes $f(h) \triangleq \sum_{i \in \mathcal{N}} \ln u_i(h)$ over all $h \in \Delta(\mathcal{H})$.
\end{definition}

As mentioned before, the proportional fairness objective has had a long history in network resource allocation literature \citep{kelly1998rate}. However, to the best of our knowledge, its applicability to the classification problem, and the implications thereof, have never been established before.

We now show that the {\PF} classifier achieves a guarantee matching the worst-case bound in Theorem \ref{thm:lowerbound}.

\begin{restatable}{theorem}{pf}
\label{thm:pf}
For any subset $g \subseteq \mathcal{N}$ that admits a perfect classifier $h^*_g \in \mathcal{H}$ (i.e., $u_g(h^*_g) = 1$) we have $u_g(h_{\PF}) \ge \frac{|g|}{|\mathcal{N}|}$.
\end{restatable}

Thus, the {\PF} classifier achieves, on any subset, an accuracy that is \emph{proportional} to the accuracy of the best classifier on that subset scaled by the fractional size of the subset. As mentioned earlier, the use of perfectly classifiable subsets in our analysis is just for the ease of exposition. The results can be suitably translated to using all possible subsets.  For example, the following is a simple corollary of \cref{thm:pf}:
\begin{restatable}{corollary}{pfcor} \label{cor:pf}
For any subset $g \subseteq \mathcal{N}$, with its best classifier $h^*_g = \arg \max_{h \in \mathcal{H}} u_g(h)$, we have $u_g(h_{\PF}) \ge \alpha \left[ u_{g}(h^*_g) \right]^2$, where $\alpha = \frac{|g|}{n}$.
\end{restatable}

Assuming black-box access to an agnostic learning oracle, the {\PF} classifier can be computed using a primal dual style algorithm (details in the Appendix, or see \citet{bhalgat2013optimal} for similar results). In our experiments, we just use a heuristic instead (see Section \ref{sec:experiments}, and also the Appendix). We also do not explicitly discuss the generalization properties -- but we would expect that {\PF} is not prone to overfitting, since all possible groups have to be given a guarantee on performance (details in the Appendix).

\paragraph{Interpreting the results:}
\cref{thm:pf} and \cref{cor:pf} neatly characterize how {\PF} achieves the best possible theoretical bound . One drawback of applying {\PF} in practice is that the theoretical guarantee is proportionally lower for smaller groups, notwithstanding the fact that, in practice, the accuracy of {\PF} on small groups is much better than what is given by these bounds (see \cref{sec:experiments}). As far as the bounds as concerned, the reason that we have to settle for an accuracy proportionally lower for smaller subsets is that the guarantee has to hold for all possible subsets. Some of these subsets could be extremely complex, and possibly unreasonable in most practical settings. As will see next, we can do much better with more restricted classes of groups.
%he same approach can be suitably adapted to somewhat more restricted classes of possible groups. 

% \subsection{{\Greedy} Classifier}\label{sec:greedy}

% We can also devise a simpler classifier that achieves similar guarantees to those given by the {\PF} classifier, namely, the iterative {\Greedy} algorithm (a more formal description is not crucial here and is deferred to the Appendix): select the classifier that classifies the most number of data points correctly, allocate it a weight proportional to this number, discard the data points that it classifies correctly, and simply repeat the above procedure until there are no data points left. The randomized classifier {\Greedy} is defined by giving to each of these classifiers a probability proportional to its weight, i.e., the number of data points classified correctly in the corresponding iteration.

%  We now show that the {\Greedy} algorithm provides a constant-factor approximation to the guarantee provided by the {\PF} classifier. Note that the first step in the \emph{while} loop of {\Greedy} (Algorithm \ref{alg:greedy}) involves using the {\ERM} agnostic learning black box. 
% \begin{restatable}{theorem}{greedy}
% \label{thm:greedy}
% If $h_{\G}$ is the {\Greedy} classifier, then for any subset $\mathcal{S} \subseteq \mathcal{N}$ that admits a perfect classifier $h_j \in \mathcal{H}$, we have $u_S(h_{\G}) \ge \frac{\alpha}{2} + \frac{1}{2 \alpha} \left(\max\left(0, 2\alpha - 1 \right) \right)^2  \ge \frac{\alpha}{2}$, where $\frac{|S|}{n} = \alpha$.
% \end{restatable}



% \begin{figure}
% \begin{minipage}{0.45\textwidth}
% \begin{algorithm}[H]
%   \caption{{\Greedy} Classifier}
%   \label{alg:greedy}
% \begin{algorithmic}
%     \STATE {\bfseries Input:} data set $\mathcal{N}$, family of classifiers  $\mathcal{H}$
%     \STATE Initialize: $r \gets 1$, $\mathcal{S}_r \gets \mathcal{N}$
%     \WHILE{$|\mathcal{S}_r| > 0$}
%         \STATE $h^*_r \gets \mbox{argmax}_{h_j} u_{\mathcal{S}_r}(h_j)$
%         \STATE $\mathcal{T}_r \gets \{i \in \mathcal{S}_r \mid u_i(h^*_r) = 1 \}$
%         \STATE $p_r \gets \frac{|\mathcal{T}_r|}{n}$
%         \STATE $\mathcal{S}_{r+1} \gets \mathcal{S}_r \setminus \mathcal{T}_r$
%         \STATE $r \gets r+1$
%     \ENDWHILE
    
%     \STATE {\bfseries Return:} classifier $h_{\G}$ that chooses $h_s^* \in \mathcal{H}$ with probability $p_s$ for $s = 1,2,\ldots,r-1$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \end{figure}  

% Therefore, for any set $\mathcal{S}$ that has a perfect classifier, the average utility of {\Greedy} is at least half the average utility of {\PF}; for large sets, the approximation factor is better, and approaches $1$ as $\alpha \rightarrow 1$. We complement our $\frac{\alpha}{2}$ analysis with Example 3 (in the Appendix) which shows that the above bound is tight when $\alpha \to 0$.

==> pf arxiv/pf_error.tex <==
%\section{{\PF} for more orderly classes of groups}\label{sec:pf_error}
\section{Best-effort guarantees for linearly separable groups}\label{sec:pf_error}
%In the previous section, we looked at a proportional guarantee on accuracy for all possible groups in the data. This led to an inevitable limitation on the worst case bounds that are theoretically achievable. 


%In recasting the proportional guarantee, we switch the quantity of interest from accuracy to error. 
In this section, we limit $\mathcal{G}$ to be a more streamlined class of groups, and aim for a much stronger guarantee. We then devise an algorithm that achieves such a guarantee. As mentioned in Section \ref{sec:model}, we want to find a a randomized classifier $h \in \Delta(\mathcal{H})$ that, for every group $g \in \mathcal{G}$, achieves an absolute error which is within an additive factor $\gamma$ from that of the optimal classifier $h^*_g$ for $g$. In particular, the optimization problem we would like to solve is the following:
\begin{problem}[{\BeFair}$(\gamma)$] For a given hypothesis space $\mathcal{H}$, a class of groups $\mathcal{G}$, and $\gamma \ge 0$,
\begin{align*}
    \min_{h \in \Delta(\hyp)} \quad & \err_{\mathcal{N}}(h) \\
\text{such that } \forall g \in \gro,  \quad &  \err_g(h^*_g) - \err_g(h) + \gamma \ge 0.
\end{align*}
\end{problem}

In particular, we consider $\mathcal{H}$ to be the space of linear hypotheses, and $\mathcal{G}$ the class of all linearly separable groups.\footnote{If $g \in \mathcal{G}$, then $g$ and $\mathcal{N} \setminus g$ are linearly separable.} As mentioned earlier, despite using linear hypotheses and groups, we are faced with a non-convex problem. It can be seen that the non-convexity stems from the best-effort constraint -- while the terms $\err_g(h)$ and $\err_g(h^*_g)$ can be individually made convex by using standard surrogate loss functions, their combination obtained by subtracting one from the other cannot. Note that such a difficulty does not arise for the more absolute notions of fairness such as \emph{parity}, as is the case with the techniques in \citet{KearnsNRW18}. Also, even in our setting, if $\mathcal{G}$ were a small finite set, then all the optimal classifiers $h^*_g$ could be calculated offline, and the corresponding constraints listed to form a simpler convex optimization problem.



We redefine the {\BeFair}($\gamma$) as follows to explicitly factor the hidden optimization problem of finding $h^*(g)$ into the corresponding constraint for $g$; by using the fact that if $\err_g(h^*_g) - \err_g(h) + \gamma \ge 0$, then $\err_g(\hpr) - \err_g(h) + \gamma \ge 0$ for any $\hpr \in {\mathcal{H}}$.

\begin{problem}[{\BeFair}$(\gamma)$]\label{prob:GPF}
\begin{align*}
    \min_{h \in \Delta(\hyp)} \quad & \err_{\mathcal{N}}(h) \\
\text{such that } \forall g \in \gro, \hpr \in \mathcal{H},  \quad &  \err_g(\hpr) - \err_g(h) + \gamma \ge 0.
\end{align*}
\end{problem}

%In the above optimization problem, we have $\err_g(h) = \sum_{i} \indicator[g(x_i) = 1] \left( 1 - u_i(h) \right)$, i.e., the absolute error accrued by $h$ over $g$. We could have equivalently written it as $\frac{\sum_{i \in \mathcal{N}}g(i)}{|\mathcal{N}|}$ (the fractional size of the group defined by $g$) times $1 - u_{g}(h)$ (the average error of $h$ on $g$). We also enforce the inequality $\err_g(h) - \err_g(\hpr) \leq \gamma$ for all possible $\hpr \in \mathcal{H}$ -- in effect, this is equivalent to enforcing it for the one value of $\hpr$ given by $\arg\min_{\hpr \in \mathcal{H}} \err_g(\hpr)$. We will shortly see why this formulation is useful.

%Note that in contrast with the previous section, the guarantee sought after is in terms of the error, and not the accuracy. We point out here that such a guarantee is stronger than the analogous one for accuracy (which can also be solved using the techniques herein).

%\paragraph{Solving the {\BeFair}($\gamma$) problem:}
We first define the partial Lagrangian corresponding to Problem \ref{prob:GPF}. Let $\phi(g,h,\hpr) \triangleq - \err_g(\hpr) + \err_g(h) - \gamma$. With dual variables $\lambda_{g, \hpr}$ for every $g \in \mathcal{G}$ and $\hpr \in \mathcal{H}$:
\begin{align*}
    L(h,\lambda) \triangleq \err(h) + \sum_{g \in \gro, \hpr \in \hyp} \lambda_{g,\hpr} \phi(g,h,\hpr).
\end{align*} 

In order to have a convergent algorithm for our optimization, we will restrict the dual space to the bounded set $\Lambda = \{\lambda \in \mathcal{R}_{+}^{ |\mathcal{G} \times \mathcal{H}|} : \Vert\lambda\Vert_1 \le C\}$, where $C$ will be a parameter in our algorithm. Then, by the Minimax Theorem, solving Problem \ref{prob:GPF} is equivalent to solving the following:
\begin{align}\label{eq:minmax}
    \min_{h \in \Delta(\hyp)} \max_{\lambda \in \Lambda}  L(h,\lambda) = \max_{\lambda \in \Lambda} \min_{h \in \Delta(\hyp)}  L(h,\lambda).
\end{align}

The minmax problem can be viewed as a two player zero-sum game: The set of pure strategies for the \emph{learner} (corresponding to the primal) corresponds to $\mathcal{H}$ -- each deterministic classifier $h \in \mathcal{H}$ is a valid pure strategy. For the \emph{adversary} (corresponding to the dual), the pure strategies in $\Lambda$ can be either the all zeros vectors, or a particular choice of $(g,\hpr) \in \mathcal{G}\times\mathcal{H}$. Then, solving Problem \ref{prob:GPF}, via the minmax formulation in Equation \ref{eq:minmax}, is the same as finding an equilibrium of the corresponding two-player zero-sum game with $L(h,\lambda)$ as the payoff for the dual player.

\subsection{Solving the {\BeFair}($\gamma$) problem via a convex relaxation:} \label{sec:solvingbefair}
The equilibrium of a two-player zero-sum game can be found using Fictitious Play, an iterative algorithm which is guaranteed to converge\footnote{The asymptotic convergence is usually fast in practice, and especially so in our experiments.} given that we can solve for the best responses of both players \citep{robinson1951iterative}. Fictitious Play \citep{brown1949some} proceeds in rounds alternating between the primal and dual player: in each round, each player chooses a best response to the the mixed strategy that randomizes uniformly over the empirical history of the other's strategies. A formal description is given in Algorithm \ref{alg:befair}.

\paragraph{Learner's best response:} For a given mixed strategy $\lambda$ of the adversary, the learner needs to solve:
\begin{align*}
    \min_{h \in \Delta(\hyp)}~ \err(h) + \sum_{g \in \gro, \hpr \in \hyp} \lambda_{g,\hpr} \err_g(h).
\end{align*}

Since the optimum is obtained at the corner points of the feasible region of the strategy space, we need only consider pure strategies for the optimization problem above. The learner's problem then becomes:
\begin{align*}
    \min_{h \in \hyp}~ \sum_i w_i \indicator[h(x_i) \neq y_i],
\end{align*}
where $w_i \triangleq 1 + \sum_{g \in \gro, \hpr \in \hyp} \lambda_{g,\hpr} \indicator[g(x_i) = 1]$, and this can be solved since we assume black-box access to a weighted {\ERM} oracle. In practice, many heuristics (like Logistic Regression, Boosting, etc.) are used effectively for this problem, even though it is known to be hard in the worst case \citep{feldman2012agnostic}.

%the primal player's best response problem is, therefore, solvable.

% \subsection{Primal player}
% The optimization problem for the primal player, given the choices of $\lambda_{g,\hpr}$, is
% \begin{align*}
%     \min_{h \in \hyp}~ \err(h) + \sum_{g \in \gro, \hpr \in \hyp} \lambda_{g,\hpr} \err_g(h).
% \end{align*}
% The objective can be written as $\sum_i w_i \indicator[h(x_i) \neq y_i]$, where
% \begin{align*}
%     w_i \triangleq 1 + \sum_{g \in \gro, \hpr \in \hyp} \lambda_{g,\hpr} \indicator[g(x_i) = 1], 
% \end{align*}
% which makes the primal player's problem equivalent to that of weighted ERM.

\paragraph{Adversary's best response:} The adversary's best response problem is more involved and will require some novel techniques to solve. Again, we need to optimize only over pure strategies. With a bit of analysis, the dual best response problem can be seen to be equivalent to solving, for a given $h \in \Delta(\mathcal{H})$:
\begin{align}\label{eqn:advprob}
    \min_{g \in \gro, \hpr \in \hyp} \err_g(\hpr) - \err_g(h).
\end{align}
For all $i \in \mathcal{N}$, define $t_i \triangleq \E \indicator[h(x_i) \neq y_i]$. Then the above objective can be written as 
\begin{align}\label{eqn:advobj}
    & \sum_i \indicator[g(x_i) = 1] \left( \indicator[\hpr(x_i) \neq y_i] -  \E \indicator[h(x_i) \neq y_i] \right) \nonumber \\
    = & \sum_i \indicator[g(x_i) \neq -1] \left( \indicator[\hpr(x_i) \neq y_i] - t_i \right),
\end{align}
which is non-convex. For each $i$, we would like to convexify it differently when $t_i = 0$ or $t_i > 0$. (The convex relaxations are not exact.)


Since we only consider the case where both $\mathcal{G}$ and $\mathcal{H}$ consist of linear hypotheses, define $z_{ig} \triangleq x_i^\intercal \theta_g$ and $z_{i\hpr} \triangleq - y x_i^\intercal \theta_{\hpr}$,
where $\theta_g$ and $\theta_{\hpr}$ are the coefficients of the linear hypotheses $g$ and $\hpr$ respectively.

For each $i \in \mathcal{N}$, we add the term $\indicator[z_{ig} > 0] \cdot \indicator[z_{i\hpr} > 0] - t_i\indicator[z_{ig} > 0]$ to the objective. The first term, $\indicator[z_{ig} > 0] \cdot \indicator[z_{i\hpr} > 0]$, is treated as $e^{z_{ig}} \cdot e^{z_{i\hpr}} = e^{z_{ig} + z_{i\hpr}}$; and the second term, $t_i\indicator[z_{ig} > 0]$, is replaced by $t_i(1 - e^{-z_{ig}})$, whence the whole objective becomes $e^{z_{ig} + z_{i\hpr}} + t_i(e^{-z_{ig}} - 1)$, which is convex.

\iffalse
We consider the cases $t_i = 0$ and $t_i > 0$ separately.


If $t_i = 0$: Each such $i \in \mathcal{N}$ adds the term $\indicator[z_{ig} > 0] \cdot \indicator[z_{i\hpr} > 0]$ to the objective. Replace each indicator function with an exponential to get $e^{z_{ig}} \cdot e^{z_{i\hpr}} = e^{z_{ig} + z_{i\hpr}}$.

If $t_i > 0$: Each such $i \in \mathcal{N}$ add the term $\indicator[z_{ig} > 0] \cdot \indicator[z_{i\hpr} > 0] - t_i\indicator[z_{ig} > 0]$ to the objective. The first term is treated as before, and the second term, $t_i\indicator[z_{ig} > 0]$, is replaced by $t_i(1 - e^{-z_{ig}})$, whence the whole objective becomes $e^{z_{ig} + z_{i\hpr}} + t_i(e^{-z_{ig}} - 1)$, which is convex.
\fi

Therefore, we need to solve 
\begin{align}\label{eqn:convexify}
    \min_{\theta_g, \theta_\hpr} \sum_{i \in \mathcal{N}} e^{z_{ig} + z_{i\hpr}} + t_i (e^{-z_{ig}} - 1),
\end{align}
which can be done via convex optimization methods.
%Using a hinge surrogate, we get
%\begin{align*}
    %&\indicator[g(x) \neq -1] \cdot \left( \indicator[\hpr(x) \neq y] - t \right) \\
    %=& \max \{0, 1 + x^\intercal \theta_g\} \cdot \max \{0, 1 - t - y x^\intercal \theta_{\hpr}\}
%\end{align*}

\begin{algorithm}[H]
   \caption{Solving {\BeFair($\gamma$)}}
   \label{alg:befair}
\begin{algorithmic}
    \STATE {\bfseries Input:} data set $\mathcal{N}$, $\gamma \ge 0$, number of rounds $T$.
    \STATE Initialize by setting $h_0$ to be some classifier in $\mathcal{H}$, and $\lambda_0$ to be the zero vector.
    \FOR{$t = 1,\ldots T$:}
        \STATE $\bar{h} \gets \mbox{uniform distribution over } \{h_0, \ldots, h_{t-1}\}$
        \STATE $\bar{\lambda} \gets \frac{1}{t}\sum_{t^\prime < t}\lambda_{t^\prime}$
        \STATE $h_t \gets$ Learner's best response to $\bar{\lambda}$
        \STATE $\lambda_t \gets$ Adversary's best response to $\bar{h}$
    \ENDFOR
    
    \STATE {\bfseries Return:} $\bar{\lambda}_t$
\end{algorithmic}
\end{algorithm}

The solution returned by Algorithm \ref{alg:befair} has to be checked for feasibility with respect to Problem \ref{prob:GPF} -- this tells us if the problem is feasible to begin with. Also, the solution to the Adversary's problem (Equation \ref{eqn:advprob}) can potentially be improved by alternately optimizing for $g$ and $\hpr$, \`a la Expectation-Maximization: For a fixed $\hpr$, we can optimize $g$ by using Equation \ref{eqn:advobj} and a convexification analogous to Equation \ref{eqn:convexify}. The converse problem of optimizing $\hpr$, for a fixed $g$, is just a weighted ERM problem.

Note that our technique works as is even for groups that can be defined in terms of any basis expansion of a limited size (a commonly used way of capturing non-linear relationships with linear methods).  For example, if there are two numerical features $x_1,x_2$, then by encoding the values $x_1^2,x_1x_2,x_2^2$ as additional features, we can solve the problem over all groups defined via conic sections (in the feature space).  Similarly, a Boolean AND of binary features can also be written as a linear constraint: for binary features $x_1,x_2$ taking values in $\{0,1\}$, $x_1 \wedge x_2$ is equivalent to $x_1 + x_2 \ge 2$. Extensions to more general classes of $\mathcal{G}$ and $\mathcal{H}$ are an interesting open problem.

\subsection{A more general version of {\BeFair}($\gamma$):} For $\delta \ge 1$, we can generalize Problem \ref{prob:GPF} as follows:
\begin{problem}[{$\delta$-\BeFair}$(\gamma)$]\label{prob:dGPF}
\begin{align*}
    \min_{h \in \Delta(\hyp)} \quad & \err_{\mathcal{N}}(h) \\
\text{such that } \forall g \in \gro,  \quad &  \delta \cdot \err_g(h^*_g) - \err_g(h) + \gamma \ge 0.
\end{align*}
\end{problem}
The only difference from Problem \ref{prob:GPF} is that we have slightly weaker constraints: the error of $h$ on $g$ is compared with $\delta$ times the least possible error on $g$. With a straightforward modification, the overall technique in Section \ref{sec:solvingbefair} works for this problem too. 

For a fixed $\delta$, computing the quantity $\max_{g \in \mathcal{G}}\err_g(h) - \delta \cdot \err_g(h^*_g)$ gives us a way of measuring the fidelity of any given classifier $h$. To do so, the Adversary's problem can be solved (as shown) to find the smallest $\gamma$ for which $h$ becomes feasible for the constraints in Problem \ref{prob:dGPF} (i.e., satisfies the best-effort guarantees). We discuss this in more detail in Section \ref{sec:pfvsbefair}. 




==> pf arxiv/problem.tex <==
\subsection{Our model and results}\label{sec:model}
We are given a set of $n$ data points denoted by $\mathcal{N}$, with their features given by $\{x_i\}_{i \in \mathcal{N}}$, and their true binary labels by $\{y_i\}_{i \in \mathcal{N}}$. The hypothesis space at hand will be denoted by $\mathcal{H}$, a set of (deterministic) classifiers. The Boolean variable $u_i(h) \in \{0,1\}$ denotes whether the classifier $h \in \mathcal{H}$ correctly classifies data point $i$. In other words, $u_i(h) = \indicator[h(x_i) = y_i]$. A classification instance is defined by a pair $(\mathcal{N}, \mathcal{H})$. 
%Note that the formulation described above captures a general multi-class classification problem, of which classification with binary labels is a special case. 
%In the binary case (with labels in $\{0,1\}$), 
We assume that for any classifier $h \in \mathcal{H}$, its \emph{complement} $\bar{h}$, defined by flipping the classification outcomes of $h$ (i.e., $h(x_i) = 1 - \bar{h}(x_i)$), is also in $\mathcal{H}$. This assumption is valid for most natural families of binary classifiers. We denote by $\Delta(\mathcal{H})$ the space of all randomized classifiers over $\mathcal{H}$. If $h \in \Delta(\mathcal{H})$ is obtained via a distribution $D_h$ over $\mathcal{H}$, then for a data point $i \in \mathcal{N}$, we defined the utility $u_i(h) \triangleq \E_{\hpr \sim D_h}[u_i(\hpr)]$.

We are given $\mathcal{G}$, a class of groups, each element of which is of the form $g : \mathcal{N} \to \{1, -1\}$. $g(i) = 1$ means $i$ is in the group and $g(i) = -1$ indicates the opposite. We also use $g$ to denote the subset given by $\{i \in \mathcal{N}: g(i) = 1\}$ and $|g|$ as its size $|\{i \in \mathcal{N}: g(i) = 1\}|$. For any such $g$, its utility under $h$ is $u_g(h) = \frac{1}{|g|} \sum_{i \in g} u_i(h)$. 

For each $g \in \mathcal{G}$, define $h^*_g \triangleq \arg \max_{h \in \mathcal{H}} u_g(h)$ to be the best classifier for the group $g$. The best-effort fairness guarantee is captured via a constraint of the form $f(u_g(h), u_g(\hpr), |g|) \ge 0$. The function $f(\cdot)$ constrains the accuracy $u_g(h)$ of $h$, the classifier at hand, to that of the optimal classifier $h^*_g$ for $g$, with a possible dependence on the size $|g|$ of the group $g$. Applying such a constraint for all $g \in \mathcal{G}$ gives us a uniform best-effort fairness guarantee. What sort of $f(\cdot)$ is workable depends on the class $\mathcal{G}$ considered. 

In Section \ref{sec:pf}, we consider the case where $\mathcal{G}$ includes all the subsets of $\mathcal{N}$, i.e., there is no specific information about $\mathcal{G}$. Via a theoretical worst-case bound (Theorem \ref{thm:lowerbound}), we show that the best we can do in this case is to choose $f(\cdot) = {u}_g(h) - \frac{|g|}{|\mathcal{N}|}[{u}_g(\hpr)]^2$. For any group $g$ that can be {\em perfectly classified} by some $\hpr \in \mathcal{H}$ ($u_g(\hpr) = 1$), the same constraint boils down to $u_g(h) \ge  |g|/|\mathcal{N}|$: in other words, a utility of at least $|g|/|\mathcal{N}|$ should be guaranteed on such a set. Such a guarantee can be interpreted as fairness: If $g$ is a potentially hidden demographic that can be perfectly classified using some features, our classifier should not ignore those features entirely. We show that our {\PF } classifier in fact achieves this guarantee (Theorem \ref{thm:pf}).

In Section \ref{sec:pf_error}, we consider a more streamlined class of groups: in particular, $\mathcal{G}$ contains all linearly separable groups. For ease of exposition, we define the error $\err_g(h) = \sum_{i \in g} [1 - u_i(h)]$, and recast the discussion in terms of it.\footnote{While a fundamentally similar discussion can be done in terms of the utilities, using errors instead leads to an easier handling of the constants involved.} In this case, we seek a much stronger guarantee: $\err_g(h) \le \err_g(h^*_g) + \gamma$. The general form of the optimization problem we solve is as follows:
\begin{align*}
    \min_{h \in \Delta(\hyp)} \quad & \err_\mathcal{N}(h) \\
\text{such that } \forall g \in \gro,  \quad &  \err_g(h^*_g) - \err_g(h) + \gamma \ge 0.
\end{align*}

As discussed in more detail later, to solve the above problem we need to deal with the non-convex constraints. We outline a method ({\BeFair}) to do so when $\mathcal{G}$ consists of linearly separable groups. We will also look for a slightly weaker guarantee as follows: $\err_g(h) \le \delta \cdot \err_g(h^*_g) + \gamma$, for some $\delta \ge 1$ -- weaker because now $\err_g(h)$ has a slightly larger target $\delta u_g(h^*_g)$ to approximate. Our techniques extend seamlessly to such a formulation also.


%The objective above is maximizing the accuracy (minimizing the error), of $h$ on the entire set $\mathcal{N}$.
% The fairness guarantees are captured by the constraints given above. On any $g \in \mathcal{G}$, the gain $u_g(h)$ of $h$ is constrained, via the function $f$ which depends on \begin{enumerate*}[label = (\alph*)]
%     \item the gain $u_g(\hpr)$ that any $\hpr \in \mathcal{H}$ could possibly achieve on $g$, and
%     \item $|g|$ (the size of $g$).
% \end{enumerate*}
% \emph{something about $f$ and how it changes}


%The restriction to perfect classification is without loss of generality, since even if $g$ cannot be perfectly classified, our guarantee will simply depend on the largest portion of $g$ that admits a perfect classification.

% In Section \ref{sec:pf_error}, we will limit consideration to a 
% collection of possible groups given by $\gro \subset \{0,1\}^\mathcal{N}$, say of a finite VC dimension. 
% For data points are indexed by $i \in \mathcal{N}$, with the features given by $x_i$ and label by $y_i$, we define for any given classifier  $h \in \mathcal{H}$, \[\err(h) \triangleq \sum_{i \in \mathcal{N}}  \indicator[h(x_i) \neq y_i] = \sum_{i} \left( 1 - u_i(h) \right). \]

% For some particular $g \in \gro$, we will define \[ \err_g(h) \triangleq \sum_{i \in \mathcal{N}} \indicator[g(x_i) = 1]\left( 1 - u_i(h) \right),\] i.e., $\err(h)$ limited to the points in $g \in \mathcal{G}$.





%In Section \ref{sec:pf}, we seek classifiers that are {\em fair} in the following sense: Consider any subset of data points $\mathcal{S}$ that can be {\em perfectly classified} by some $h_j \in \mathcal{H}$ ($u_i(h_j) = 1$ for all $i \in \mathcal{S}$). Our classifier should guarantee some non-trivial average utility to $\mathcal{S}$ that degrades with $|\mathcal{S}|$. The restriction to perfect classification is without loss of generality, since even if $\mathcal{S}$ cannot be perfectly classified, our guarantee will simply depend on the largest portion of $\mathcal{S}$ that admits a perfect classification. Such a guarantee can be interpreted as fairness: If $\mathcal{S}$ is a potentially hidden demographic that can be perfectly classified using some features, our classifier should not ignore those features entirely. 

%On the other hand, when $\mathcal{S}$ is large and adversarially chosen, and the points not in $\mathcal{S}$ have been corrupted, this will imply a {\em robustness} guarantee, where the classifier provides a non-trivial guarantee on the utility provided to the unknown true data set $\mathcal{S}$.

%In many applications, data points can be inaccurate or even adversarially tainted, which renders the na\"{i}ve solution that maximizes the sum of utilities potentially undesirable. We aim for a robust algorithm $\mathsf{A}$ to get a theoretical guarantee on the performance $\mathsf{A}(\mathcal{S}) := \frac{1}{|\mathcal{S}|} \cdot \sum_{i \in \mathcal{S}} u_i(h_\mathsf{A})$ where $h_\mathsf{A}$ is the (randomized) classifier returned by the algorithm. For \emph{any} subset $\mathcal{S} \subseteq \mathcal{N}$ of data points, we compare with the benchmark performance $\gamma(\mathcal{S})$ achieved by maximizing the sum of utilities on this set $\mathcal{S}$, \emph{i.e.}, $\gamma(\mathcal{S}) = \frac{1}{|\mathcal{S}|} \cdot \max_{h_j \in \mathcal{H}} \sum_{i \in \mathcal{S}} u_i(h_j)$.



==> pf arxiv/related.tex <==
\subsection{Related literature}
\label{sec:related}
The extant literature on fairness in machine learning \cite{hardt2016equality, kamiran2012data, hajian2012methodology, chouldechova2017fair, corbett2017algorithmic} primarily considers statistical notions of fairness which require the protected groups to be specified as input to the (binary) classification problem. Many of these notions are further known to be incompatible with one another \cite{kleinberg2018inherent, friedler2016possibility}. Individual notions of fairness, which loosely translate to asking for ``similar individuals'' to be ``treated similarly'', have also been studied \cite{dwork2012fairness}. However, this requires additional assumptions to be made about the problem at hand, in the form of, e.g., a ``similarity metric'' defined on pairs of data points. Another related notion is envy-freeness \citep{HossainMS19}, which isn't very useful without group information (more in the Appendix).


There are several papers on fairness that utilize the broadly applicable framework of minimax optimization in their algorithms \citep{agarwal2018reductions, rezaei2020fairness, baharlouei2019renyi, madras2018learning}.
For example, \cite{rezaei2020fairness} derive a novel distributionally robust classification method by incorporating fairness criteria into a worst-case loss minimization program. When compared with this literature, our work is different in one or both of two senses: First, we have a novel and conceptually different notion of fairness that approximates the best-effort guarantee for each group, as opposed to objectives such as max-min fairness or parity. Second, the cardinality of the set of groups can be unbounded (defined by linear constraints on either the feature space or its basis expansion) in our case, as opposed to operating with a fixed set of groups. As we shall see later, each of these aspects presents its own technical challenges.


Several issues have been raised with respect to defining the demographic groups that need to be considered for fairness. \cite{chen2019fairness} assess the prevalence of disparity when missing demographic identities are imputed from the data. \cite{hashimoto2018fairness} look at a model where user retention among different groups is linked to the accuracy achieved on them respectively, and design algorithms that improve the user retention among minority groups based on distributionally robust optimization. Their methods, while oblivious to the identity of the groups, operate under the assumption that there are a fixed number $K$ of groups, and work well in practice for small $K$. \citep{kim2019multiaccuracy} develop multi-accuracy auditing to guarantee the fairness for identifiable subgroups, by post-processing the classifier such that it is unbiased. \cite{KearnsNRW18} study the problem of auditing classifiers for statistical parity (or other related fairness concepts) across a (possibly infinite) collection of groups of bounded VC dimension. However, they do not consider the fact that some groups could be inherently harder to classify than others, and instead work with standard statistical notions such as statistical parity. Doing so results in a non-convex problem -- something that we deal with in our work. 

%Another drawback of standard approaches to fairness is that they primarily apply to the case of binary classification, with little work on generalizing them to the multi-class setting \citep{heidari2019moral, HossainMS19}. All our methods extend to the multi-class setting with little or no modification. 

Our {\BeFair} approach assumes black-box access to an agnostic learning oracle. Such reductions are commonplace in recent work on fairness in machine learning \citep{KearnsNRW18}. For example, \cite{agarwal2018reductions} reduce fair classification to a sequence of cost-sensitive classifications, the solutions of which can be achieved using out-of-the-box classification methods. 

The study of fairness has had a much longer history in economics, in particular, the literature on fair division and cake-cutting \citep{brams1996fair, robertson1998cake}. Out of this line of work have emerged general notions of fairness such as proportionality \citep{steinhaus1948problem}, envy-freeness \citep{varian1973equity}, the core \citep{foley1970lindahl}, and egalitarian (or maxmin) fairness \citep{rawls2009theory, hahne1991round}, to name a few. Of these, the idea of envy-freeness has received great attention in computer science (e.g., \citep{chen2013truth, cohler2011optimal}), and been amenable to adaptation into machine learning as a group-based notion of fairness \citep{balcan2019envy, ustun2019fairness, zafar2017parity}. \citet{HossainMS19} devise algorithms, for multi-class classification that can achieve a variant of group-based (approximate) envy-freeness, with sample complexity of the order of $\log |\mathcal{G}|$, where $\mathcal{G}$ is the collection of pre-defined groups. Our guarantees on the accuracy of the {\PF} classifier are related to the notion of the core: for example, analogous guarantees have been studied in the setting of participatory budgeting \citep{fain2016core}. However, dealing with envy-freeness at an individual level, in the absence of group information, is not very useful. Even in simple binary settings, such as loan and bail applications (all individuals prefer being classified positively, i.e. receiving a loan/bail), satisfying envy-freeness requires all individuals to receive the same outcome \citep{HossainMS19}.

Practical implementations of the above-mentioned economic notions of fairness have garnered interest in the literature on network resource allocation \citep{kleinberg1999fairness, kumar2006fairness}. Proportional fairness \citep{kelly1998rate, bonald2006queueing} has been seen as a way of attaining a middle-ground between welfare maximization and maxmin fairness \citep{jain1984quantitative}. The applicability of proportional fairness to machine learning, in terms of the performance of classification across groups, has, to the best of our knowledge, not been studied before. Although, \cite{li2019fair} do study fair resource allocation based on $\alpha$-fairness (of which proportional fairness is a special case with $\alpha=1$) to improve fairness in terms of the performance across devices in a decentralized federated learning setting.
%{\color{red} Zhihao: Are these works violate our claim that the applicability of proportional fairness to machine learning have not been studied before? They do not exactly use the proportional fairness, but they use $\alpha$-fairness, where proportional fairness is a special case of $\alpha$-fairness. Also, please help me to check whether the added things are appropriate.}




==> pf arxiv/settings.tex <==
\usepackage{indentfirst}
\usepackage{amsmath, amssymb, amsthm, amsfonts}
\usepackage{xcolor}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{paralist}
\usepackage{xurl}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{diagbox}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{claim}{Claim}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{example}{Example}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\definecolor{colorx}{rgb}{0.4, 0.1, 0.7}
\newcommand{\kn}[1]{\textcolor{colorx}{[Kangning: #1]}}
\newcommand{\yu}[1]{\textcolor{colorx}{[Yu: #1]}}

\newcommand{\eps}{{\varepsilon}}
\newcommand{\Greedy}{\textsc{Greedy}}
\newcommand{\Ada}{\textsc{Ada}}
\newcommand{\LR}{\textsc{LR}}
\newcommand{\PF}{\textsc{PF}}
\newcommand{\hPF}{\textsc{hPF}}
\newcommand{\ERM}{\textsc{ERM}}
\newcommand{\BeFair}{\textsc{BeFair}}
\newcommand{\G}{\textsc{G}}

\newcommand{\mae}{\mathrm{MAE}}

\newcommand{\Fair}{{\sc\texttt{Fair}}}

\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}
\usepackage[capitalise]{cleveref}

\usepackage[symbol]{footmisc}
\usepackage{wrapfig}

%\usepackage{appendix}
%\renewcommand{\appendixname}{Part}

\usepackage{multibib}
\newcites{SM}{Supplementary References}

%%%%%%%%%%%%%%%%%
\usepackage{bbm}
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\indicator}{\mathbbm{1}}
\newcommand{\E}{\mathbbm{E}}
\newcommand{\gro}{\mathcal{G}}
\newcommand{\hyp}{\mathcal{H}}
\newcommand{\hpr}{{h^\prime}}
%\newcommand{\zg}{z_g}
%\newcommand{\zhpr}{z_\hpr}

\usepackage[inline]{enumitem}
